Aligning language models with human preferences

Language models (LMs) trained on vast quantities of text data can acquire sophisticated skills such as generating summaries, answering questions or generating code. However, they also manifest behaviors that violate human preferences, e.g., they can generate offensive content, falsehoods or perpetuate social biases. In this thesis, I explore several approaches to aligning LMs with human preferences. First, I argue that aligning LMs can be seen as Bayesian inference: conditioning a prior (base, pretrained LM) on evidence about human preferences (Chapter 2). Conditioning on human preferences can be implemented in numerous ways. In Chapter 3, I investigate the relation between two approaches to finetuning pretrained LMs using feedback given by a scoring function: reinforcement learning from human feedback (RLHF) and distribution matching. I show that RLHF can be seen as a special case of distribution matching but distributional matching is strictly more general. In chapter 4, I show how to extend the distribution matching to conditional language models. Finally, in chapter 5 I explore a different root: conditioning an LM on human preferences already during pretraining. I show that involving human feedback from the very start tends to be more effective than using it only during supervised finetuning. Overall, these results highlight the room for alignment techniques different from and complementary to RLHF.

==> figures/chapter3/tab_RLvsDPG.tex <==

\begin{table*}[t]
    \centering
    \small
    \vspace{-0.5cm}
\begin{tabular}{lll}
\toprule
 & \textbf{Policy Gradients} & \textbf{\DPG}\\
\midrule
 \textbf{Reward} & 
 $R(x)$   & 
 $R_\theta(x) =\frac{P(x)}{\pi_\theta(x)}$ \\
 \addlinespace
%   \textbf{Advantage} & 
%  $R(x) - [\E_{x \sim\pit} R(x)]$ & 
%  $\frac{P(x)}{\pi_\theta(x)} - Z$ \\
 \textbf{ $\nabla_\theta$} & 
{\small $\E_{x \sim \pit} R(x) \nabt \log \pit(x)$} & 
{\small $\E_{x \sim \pit} \frac{P(x)}{\pi_\theta(x)} \nabt \log \pit(x)$} \\
 \addlinespace
 \textbf{Baseline}& 
 $\E_{x \sim\pit} R(x)$  & 
 $Z$   \\
\addlinespace
 \textbf{ $\nabla_\theta$ with Baseline } & 
 {\small $\E_{x \sim \pit} \Big[R(x) - \E_{x \sim\pit} R(x) \Big] \nabt \log \pit(x)$} & 
{\small $\E_{x \sim \pit} \Big[ \frac{P(x)}{\pi_\theta(x)} - Z \Big] \nabt \log \pit(x)$} \\
\bottomrule
\end{tabular}
    \caption{\small{A comparison between Policy Gradients~\citep{sutton_policy_gradients} and Distributional Policy Gradients~\citep{opt-rl-arxiv-2019} forms of Reward, Baseline, and Gradient of the loss function (the PG-term) before ($\nabla_\theta$) and after ($\nabla_\theta$ with Baseline) including a baseline for variance reduction .}}
    \label{tab:comparison_DPGvsPG}
\end{table*}

==> figures/chapter3/table_bsz_experiments.tex <==
\begin{table}
\tiny
\begin{tabular}{lllrrrrrrrrr}
\toprule
             &      &      &  b(x) &  KL(p, pi) &  KL(pi, a) &  Dist-1 &  Dist-2 &  Dist-3 &  SB-3 &  SB-4 &  SB-5 \\
             & batch size & method &      &        &        &       &       &       &        &        &        \\
\midrule
word amazing & 0    & a & 0.00 &   6.46 &  -0.00 &  0.87 &  0.95 &  0.93 &   0.96 &   0.90 &   0.82 \\
             & 256  & GDC++ & 0.72 &   3.94 &   7.28 &  0.87 &  0.95 &  0.94 &   0.97 &   0.94 &   0.88 \\
             &      & GDC & 0.59 &   4.61 &   8.34 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             \
             & 512  & GDC++ & 0.72 &   2.57 &   5.34 &  0.86 &  0.95 &  0.93 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.69 &   2.40 &   5.36 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             & 1024 & GDC++ & 0.75 &   1.34 &   4.71 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.73 &   1.89 &   4.70 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             & 2048 & GDC++ & 0.73 &   1.35 &   4.33 &  0.87 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
             &      & GDC & 0.71 &   1.46 &   4.40 &  0.86 &  0.95 &  0.94 &   0.97 &   0.93 &   0.87 \\
\bottomrule
Multiple Dist & 0    & a & 0.12 &   0.16 &   0.00 &  0.90 &  0.95 &  0.92 &   0.98 &   0.94 &   0.90 \\
             & 256  & GDC++ & 0.24 &   0.65 &   1.06 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.23 &   0.52 &   1.04 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 512  & GDC++ & 0.24 &   0.37 &   0.78 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.23 &   0.36 &   0.88 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 1024 & GDC++ & 0.24 &   0.20 &   0.75 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.24 &   0.24 &   0.81 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\
             & 2048 & GDC++ & 0.24 &   0.20 &   0.68 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.91 \\
             &      & GDC & 0.24 &   0.22 &   0.70 &  0.90 &  0.95 &  0.92 &   0.98 &   0.95 &   0.90 \\

\bottomrule
\end{tabular}
\end{table}


==> figures/chapter3/table_pointwise_dist_experiments.tex <==
\begin{table}[H]
\tiny
\centering
\begin{tabular}{llcccccccc}
\toprule
 &   &  &  \multicolumn{2}{c}{\textbf{Fluency}} & \multicolumn{3}{c}{\textbf{Sentence Level Diversity}} &  \multicolumn{2}{l}{\textbf{Corpus Level Diversity}} \\
& \textbf{Method}  &  \textbf{Ctrl ($\uparrow$)} & \textbf{KL{(p,$\boldsymbol{\pi}$)}} ($\downarrow$) &  \textbf{KL(pi,a)} ($\downarrow$)&  \textbf{Dist-1} ($\uparrow$)&  \textbf{Dist-2} ($\uparrow$)&  \textbf{Dist-3} ($\uparrow$)&  \textbf{SB-4} ($\downarrow$)&  \textbf{SB-5}($\downarrow$) \\
\midrule
\multicolumn{10}{c}{\textbf{Pointwise Constraints Experiments}}\\
\midrule
Word Amazing 
 & \gc{Original LM} &  \gc{0.00} &  \gc{6.02} &  \gc{0.00} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &  \gc{0.89} &  \gc{0.82} \\
 & Reinforce &  \r{1.00} &  \r{134.31} & \r{78.39} &  \r{0.69} &  \r{0.91} &  \r{0.94} &  \r{0.98} &  \r{0.96} \\
 & Ziegler &  \textbf{0.82} &  4.56 &  5.88 &  0.86 &  0.95 &  0.94 &  0.94&  0.88 \\
 & GDC &  0.65 &  2.57 &  5.06 &  0.86 &  0.95 &  0.94 &  0.93 &  0.87 \\
 & GDC++ (Ours)&  \underline{0.69} &  \underline{\textbf{2.10}} &  \underline{\textbf{4.74}} &  \underline{\textbf{0.87}} &  0.95 &  0.94 &  0.93 &  0.87 \\
   \midrule
Word WikiLeaks 
 & \gc{Original LM} &  \gc{0.00} &  \gc{8.54} &  \gc{0.00} &  \gc{0.86} &  \gc{0.9}4 &  \gc{0.92} &  \gc{0.89} &  \gc{0.80} \\
 & Reinforce &  \r{1.00}&  \r{8.00} &  \r{117.24} &  \r{0.38} &  \r{0.56} & \r{0.64} & \r{0.98} &  \r{0.97} \\
 & Ziegler &  0.68 &  0.00 &  6.03 &  0.87 &  0.96 &  0.94 &  0.95 &  0.90 \\
 & GDC &  0.75 &  3.22 &  7.96 &  0.88 &  0.96 &  0.94 &   0.95 &  0.90 \\
 & GDC++ (Ours) &    \underline{\textbf{0.77}} &  \underline{\textbf{2.21}} &  \underline{\textbf{7.53}} &  0.88 &  0.96 &  0.94 &  0.95 &  0.91 \\
  \midrule
Wordlist Science 
 & \gc{Original LM} &  \gc{0.06} & \gc{2.79} & \gc{0.00} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &  \gc{0.89} &  \gc{0.81} \\
 & Reinforce&  \r{1.00} &  \r{140.02} &  \r{66.68} &  \r{0.29} &  \r{0.41} &  \r{0.49} & \r{0.98} &   \r{0.97} \\
  & Ziegler &  \textbf{1.00} &    6.1 &  5.88 &  0.86 &  0.95 &  0.93 &  0.95 &  0.90\\
 & GDC &  0.52 &  2.27 &  2.89 &  0.86 &  0.95 &  0.93 &  0.93 &  0.87 \\
 & GDC++ (Ours) &  \underline{0.54} &  \underline{1.78} &  \underline{\textbf{2.11}} &  0.86 &  0.95 &  0.93 & \underline{\textbf{0.92}} &  \underline{\textbf{0.86}} \\
  \midrule
Wordlist Politics 
 & \gc{Original LM} &  \gc{0.07} &  \gc{2.65} &  \gc{0.01} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &  \gc{0.89} &  \gc{0.81} \\
 & Reinforce&  \r{1.00} &  \r{263.79} &  \r{65.06} &  \r{0.26} &  \r{0.40} &  \r{0.51}& \r{0.98} &  \r{0.97} \\
 & Ziegler &  \textbf{1.00} &  8.46 &  5.92 &  0.87 &  0.96 &  0.94 &  0.96 &  0.92 \\
 & GDC &  \underline{0.58} &  2.70 &  2.49 &  0.87 &  \underline{0.96} &  \underline{0.94} &  0.93 &  0.88 \\
 & GDC++ (Ours) &  0.49 &  \underline{\textbf{2.01}} &  \underline{\textbf{1.35}} &  0.87 &  0.95 &  0.93 &  0.93 &  \underline{\textbf{0.87}} \\
  \midrule
+ve Sentiment 
 & \gc{Original LM} &  \gc{0.17} &  \gc{2.06} &  \gc{0.01} &  \gc{0.86} &  \gc{0.94} &  \gc{0.93} &  \gc{0.89} &  \gc{0.81} \\
 & Reinforce &  \r{1.00} &  \r{153.75} &  \r{80.07} &  \r{0.27} &  \r{0.37} &  \r{0.41} &  \r{0.97} &  \r{0.95} \\
 & Ziegler &  \textbf{0.98} &  5.70 &  5.98 &  0.85 &  0.96 &  0.94 &   0.96 &  0.91 \\
 & GDC &  0.59 &  1.68 &  1.89 &  0.86 &  0.95 &  0.94 &  0.93 &  0.87 \\
 & GDC++ (Ours) &  \underline{0.60} &  \underline{\textbf{1.67}} &  \underline{\textbf{1.88}} &  0.86 &  0.95 &  0.94 &  0.93 &  0.87 \\
  \midrule
-ve Sentiment 
 & \gc{Original LM} &  \gc{0.13} &  \gc{2.14} &  \gc{0.01} &  \gc{0.86} &  \gc{0.94} &  \gc{0.92} &   \gc{0.90} &  \gc{0.82} \\
 & Reinforce &  \r{1.00} &  \r{88.48} &  \r{70.38} &  \r{0.83} &  \r{0.96} &  \r{0.94} &  \r{0.97} &  \r{0.93} \\
 & Ziegler &  0.95 &  6.12 &  6.00 &  0.84 &  0.95 &  0.94 &  0.96 &  0.92 \\
 & GDC &  \underline{0.52} &  1.72 &  1.79 &  0.86 &  0.95 &  0.94 &  0.94 &  0.88 \\
 & GDC++ (Ours) &  0.51 &  \underline{\textbf{1.66}} &  \underline{\textbf{1.63}} &  0.86 &  0.95 &  0.94 & \underline{\textbf{0.93}} &  0.88 \\
  \midrule
  \multicolumn{10}{c}{\textbf{Distributional Constraints Experiments}}\\
  \midrule
Single 
 & \gc{Original LM} &  \gc{0.19} &  \gc{0.39} &  \gc{0.01} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.90} \\
 & GDC &  0.80 &  0.74 &  0.71 &  0.89 &  0.95 &  0.92 &  0.95 &  0.90 \\
 & GDC++ (Ours) &  \underline{\textbf{0.81}} &  \underline{\textbf{0.33}} &  \underline{\textbf{0.66}} &  0.89 &  0.95 &  0.92 &  \underline{\textbf{0.94}} &  0.90 \\
  \midrule
Multiple 
 & \gc{Original LM} &  \gc{0.49} &  \gc{0.40} &  \gc{0.00} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.90} \\
 & GDC &  0.92 &  0.53 &  0.85 &  0.90 &  0.95 &  0.92 &  0.95 &  0.90 \\
 & GDC++ (Ours) &  \underline{\textbf{0.95}} &  \underline{\textbf{0.30}} &  \underline{\textbf{0.76}} &  0.90 &  0.95 &  0.92 &  0.95 &  0.90 \\
  \midrule
Hybrid Sports 
 & \gc{Original LM} &  \gc{0.22} &  \gc{0.20} &  \gc{0.00} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.90} \\
 & GDC &  \underline{\textbf{0.87}} &  \underline{\textbf{0.24}} &  2.65 &  0.93 &  0.95 &  0.92 &  0.96 &  0.92 \\
 & GDC++ (Ours) &  0.85 &  0.87 &  \underline{\textbf{2.35}} &  0.93 &  0.95 &  0.92 &  0.96 &  0.92 \\
  \midrule
Hybrid Science 
 & \gc{Original LM} &  \gc{0.09} &  \gc{0.00} &  \gc{0.00} &  \gc{0.90} &  \gc{0.95} &  \gc{0.92} &  \gc{0.94} &  \gc{0.89} \\
 & GDC &  0.68 &  1.52 &  3.92 &  0.88 &  0.95 &  0.91 &  0.95 &  0.92 \\
 & GDC++ (Ours) &  \underline{\textbf{0.70}} &  \underline{\textbf{1.41}} &  \underline{\textbf{3.83}} &  0.88 &  0.95 &  \underline{\textbf{0.92}} &  0.95 &  \underline{\textbf{0.91}} \\
%   \midrule
% avg & GDC &  0.55 &  1.74 &  2.92 &  0.88 &  0.95 &  0.93 &  0.97 &  0.94 &  0.89 \\
%  & GDC++ (Ours) &  0.54 &  1.43 &  2.68 &  0.88 &  0.95 &  0.93 &  0.97 &  0.94 &  0.89 \\
%  & Original LM &  0.09 &  2.52 &  0.00 &  0.88 &  0.95 &  0.92 &  0.96 &  0.91 &  0.85 \\
%  & Reinforce &  1.00 &  131.39 &  79.64 &  0.45 &  0.60 &  0.65 &  0.99 &  0.98 &  0.96 \\
%  & Ziegler &  0.89 &  4.97 &  5.96 &  0.86 &  0.96 &  0.94 &  0.98 &  0.95 &  0.91 \\
\bottomrule
\vspace{5px}
\end{tabular}
\caption{
\small{
%   Evaluation metrics:  $\KL(p, \pi_{\theta})$ ($\downarrow$ better), $\mathbb{E}_{\pit} \phi(x)$ ($\uparrow$ better), $\KL(\pi_{\theta}, a)$ ($\downarrow$ better), Self-BLEU-5 ($\downarrow$ better), and Distinct-1 ($\uparrow$ better) aggregated over 6 pointwise constraints experiments (tasks 1-6) for policies obtained from GDC\texttt{++}, GDC, Ziegler and Reinforce. See Figure~\ref{fig:distributional-compare-methods-metrics} for aggregated distributional constraints experiments, and Figures \ref{fig:pointwise-compare-methods-split1}-\ref{fig:distributional-compare-methods-split} in the Appendix for a detailed view on each experiment.
      Evaluation over 6 pointwise constraints experiments (tasks 1-6) and 4 distributional constraints experiments (tasks 7-10) for policies obtained from GDC\texttt{++} (ours), GDC, Ziegler and Reinforce.
      See figures \ref{fig:pointwise-compare-methods-split1}-\ref{fig:distributional-compare-methods-split} in the Appendix for a detailed view on each experiment.
    %   $\KL(p, \pi_{\theta})$ ($\downarrow$ better), $\mathbb{E}_{\pit} \phi(x)$ ($\uparrow$ better), $\KL(\pi_{\theta}, a)$ ($\downarrow$ better), Self-BLEU-5 ($\downarrow$ better), and Distinct-n ($\uparrow$ better).
      Results of the initial policy (\gc{Original LM}) are displayed for reference.The best method (excluding ties) overall is highlighted in \textbf{bold}, while the best method between GDC and GDC++ is \underline{underlined}. Runs that suffer degeneration due to \r{catastrophic forgetting} (measured by sequence level repetitions) are highlighted in red and excluded from best method comparison. Our method GDC++ that includes a baseline for variance reduction, outperforms GDC \citep{khalifa_2021} in 7/10 tasks in terms of control satisfaction rate (\textbf{Ctrl}), as well as convergence towards the optimal policy (\textbf{KL{(p,$\boldsymbol{\pi}$)}}) and distance from the original LM (\textbf{KL(pi,a)}) in 10/10 of the tasks. 
   }
   }
   \label{tab:all_experiments_results}
\end{table}


